PARASIDE: An Automatic Paranasal Sinus Segmentation and Structure Analysis Tool for MRI

Chronic rhinosinusitis (CRS) is a common and persistent sinus imflammation that affects 5 - 12\% of the general population. It significantly impacts quality of life and is often difficult to assess due to its subjective nature in clinical evaluation. We introduce PARASIDE, an automatic tool for segmenting air and soft tissue volumes of the structures of the sinus maxillaris, frontalis, sphenodalis and ethmoidalis in T1 MRI. By utilizing that segmentation, we can quantify feature relations that have been observed only manually and subjectively before. We performed an exemplary study and showed both volume and intensity relations between structures and radiology reports. While the soft tissue segmentation is good, the automated annotations of the air volumes are excellent. The average intensity over air structures are consistently below those of the soft tissues, close to perfect separability. Healthy subjects exhibit lower soft tissue volumes and lower intensities. Our developed system is the first automated whole nasal segmentation of 16 structures, and capable of calculating medical relevant features such as the Lund-Mackay score.

==> artwork.tex <==
\section{Artwork}
\label{artwork}

==> conclusions.tex <==
\section{Discussion}
\label{discussion}

%The discussion section should explore the significance of your results but not repeat them. You may combine your results and discussion sections into one section, if appropriate. We recommend that you avoid the use of extensive citations and discussion of published literature in the discussion section.


%The conclusion section should present the main conclusions of your study. You may have a stand-alone conclusions section or include your conclusions in a subsection of your discussion or results and discussion section.

–	Summary-statement of the study

–	Competitors (related work), why are we better/worse than they, highlighting our strenghts



–	Limitations of our study


–	Clinical relevance



–	Conclusion


==> tab_pathdetection.tex <==
%& Densenet169+Seg
\begin{table}[hbpt]
    \centering
    \small
    \begin{tabular}{lcccc}
        \toprule
        Model               & V. maxillaris     & V. frontalis      &  V. sphenoidalis  & V. ethmoidalis\\
        \midrule
        Densenet169         & $0.66 \pm 0.1$    & $0.35 \pm 0.1$    & $0.22 \pm 0.1$    & $0.47 \pm 0.1$\\
        Resnet18            & $0.01 \pm 0.1$    & $0.01 \pm 0.1$    & TBD               & $0.01 \pm 0.1$\\
        Densenet169+BinSeg     & $0.01 \pm 0.1$    & $0.01 \pm 0.1$    & TBD               & $0.01 \pm 0.1$\\
        nnUNet (ours)       & TBD               & TBD               & TBD               & $0.01 \pm 0.1$\\
        nnUNet+post (ours)  & TBD               & TBD               & TBD               & $0.01 \pm 0.1$\\
        %\midrule
        %Average  & TBD & TBD & TBD & $0.01 \pm 0.1$\\
        \bottomrule
    \end{tabular}
    \caption{Pathology detection using different approaches. Values are the F1-score, mean and standard deviation are reported. The higher the value, the better. Best values for each structure is marked in bold.}
    \label{tab:detection}
\end{table}

% Denset169, 56 [0.6618704795837402, 0.6554216742515564, 0.3534482717514038, 0.3404255211353302, 0.22516556084156036, 0.22077922523021698, 0.4738955795764923, 0.47580644488334656]
% Resnet18, 7 
